Finite Element Analysis of the Schroedinger Equation

The purpose of this work is to test the application of the finite element method to quantum mechanical problems, in particular for solving the Schroedinger equation. We begin with an overview of quantum mechanics, and standard numerical techniques. We then give an introduction to finite element analysis using the diffusion equation as an example. Three numerical time evolution methods are considered: the (tried and tested) Crank-Nicolson method, the continuous space-time method, and the discontinuous space-time method.

==> IndependentSchrodinger.tex <==
\chapter{Time-Independent Analysis}
\label{IndependentSchrodinger} 
In this chapter we will construct the discretized mathematical model of the time independent \schro equation,
\begin{equation}
-\frac{\hbar^2}{2m}\frac{d^2\psi}{dx^2}+V(x)\psi=E\psi.
\end{equation}
The main aim of this part of the work is to determine the energy level configurations for particles in various potentials.  We will first consider a particle in an infinite well where $V=0$, this will then be extended to a general well $V(x)$.    

\section{Model of Infinite Potential Well}
To model an infinite potential well using FEM we begin with the \schro equation with zero potential,
\begin{equation}
\frac{d^2\psi}{dx^2}+\gamma\psi=0
\end{equation}
where $\gamma=\frac{2mE}{\hbar^2}$.  Now using the FEM construction described in Sec.~\ref{eigen-value} we obtain the \schro equation FE approximation:
\begin{equation}
\sum_e \left\{
\left[
\begin{array}{cc}
	1 & -1 \\
	-1 & 1 \\
\end{array}
\right]-
\frac{l_e^2 \gamma}{6}
\left[
\begin{array}{cc}
	2 & 1 \\
	1 & 2 \\
\end{array}
\right]
\right\}
\bar{\psi}=0
\label{schro-time-ind}
\end{equation}
From the boundary conditions of an infinite potential well we know that the nodal approximations at the edges of the well are zero: $\psi_1=\psi_{N+1}=0$ (where $N$ is the number of elements).  Therefore, assembling for $N$ elements we have the generalized eigenvalue problem:
\begin{equation}
\left\{
\left[
\begin{array}{ccccc}
	2 & -1 & 0 &  \cdots & 0  \\
	-1 & 2 & -1 & & \vdots  \\
	0 & -1 & 2 &   & 0  \\
  \vdots &  &  & \ddots & -1 \\
  0 & \cdots & 0 & -1 & 2 \\
\end{array}
\right]-
\frac{l_e^2 \gamma}{6}
\left[
\begin{array}{ccccc}
	4 & 1 & 0 &  \cdots & 0  \\
	1 & 4 & 1 & & \vdots  \\
	0 & 1 & 4 &   & 0  \\
  \vdots &  &  & \ddots & 1 \\
  0 & \cdots & 0 & 1 & 4 \\
\end{array}
\right]
\right\}
\left[
\begin{array}{c}
	\psi_2  \\
  \psi_3  \\
  \psi_4	\\
	 \vdots \\
   \psi_{N} \\
\end{array}
\right]
=\textbf{0}
\label{time-independent-no-potential-equation}
\end{equation}

\section{Model of a General Potential $V(x)$}
To take into account a general potential we need to model
\begin{equation}
\frac{d^2\psi}{dx^2}-V(x)\psi+\gamma\psi=0.
\end{equation}
The extra potential term is incorporated through the following FE approximation
\begin{equation}
\sum_e\frac{2m\bar{V}_e}{\hbar^2}\left(\int^1_{-1}\textbf{N}^{\dagger}\textbf{N}d\xi\right)\bar{\psi}=\sum_e\frac{m l_e\bar{V}_e}{\hbar^2}
\left[
\begin{array}{cc}
	2 & 1 \\
	1 & 2 \\
\end{array}
\right]
\bar{\psi}
\end{equation}
where $\bar{V}_e$ is the average potential within the element $e$.  Assembling for $N$ elements we obtain the full \schro FE approximation:
\begin{equation}
\textbf{0}=\left\{\textbf{A}+\frac{ml_e^2}{\hbar^2}\textbf{B}-\frac{l_e^2 \gamma}{6}\textbf{C}\right\}\bar{\psi}
\end{equation}
where the matrices are given as:
\begin{eqnarray}
\textbf{A}&=&\left[
\begin{array}{ccccc}
	1 & -1 & 0 &  \cdots & 0  \\
	-1 & 2 & -1 & & \vdots  \\
	0 & -1 & 2 &   & 0  \\
  \vdots &  &  & \ddots & -1 \\
  0 & \cdots & 0 & -1 & 1 \\
\end{array}
\right],\nonumber\\
\textbf{B}&=&
\left[
\begin{array}{ccccc}
	\bar{V}_1 & -\bar{V}_1 & 0 &  \cdots & 0  \\
	-\bar{V}_1 & \bar{V}_1+\bar{V}_2 & -\bar{V}_2 & & \vdots  \\
	0 & -\bar{V}_2 & \bar{V}_2+\bar{V}_3 &   & 0  \\
  \vdots &  &  & \ddots & -\bar{V}_N \\
  0 & \cdots & 0 & -\bar{V}_N & \bar{V}_N \\
\end{array}
\right],\nonumber\\
\textbf{C}&=&
\left[
\begin{array}{ccccc}
	2 & 1 & 0 &  \cdots & 0  \\
	1 & 4 & 1 & & \vdots  \\
	0 & 1 & 4 &   & 0  \\
  \vdots &  &  & \ddots & 1 \\
  0 & \cdots & 0 & 1 & 2 \\
\end{array}
\right],
\end{eqnarray}
and the nodal vector is
\begin{equation}
\bar{\psi}=
\left[
\begin{array}{c}
	\psi_1  \\
  \psi_2  \\
  \psi_3	\\
	 \vdots \\
   \psi_{N+1} \\
\end{array}
\right].
\end{equation}

\section{Results}

==> timepotential.tex <==
\chapter{Time Varying Potential $V(x,t)$}
\label{timepotential}
In this chapter we will apply the Crank-Nicholson/Finite-Element method to a particle in an infinite potential well, where at at time $t'$ a sinusoidal time varying potential will be turned on:
\begin{equation}
V(x,t)=A \sin\left[k x - w t\right],
\label{time-varying-potential}
\end{equation}
where $A$ is the field amplitude, $k$ is the wave number, and $\omega$ is the angular frequency.
\section{Construction of the model}
In order to incorporate the time varying potential into the Crank-Nicholson method we need to recalculate the potential term in Eqn.~(\ref{standard-potential}), but this time by taking into account the potential in Eqn.~(\ref{time-varying-potential}).  We therefore have
\begin{eqnarray}
-\frac{i}{\hbar}\int^L_0 V(x,t)\phi \psi dx&=&-\frac{i}{2\hbar}\sum_e l_e \int^{1}_{-1}\bar{\phi}^{\dagger}V(\xi,t)\textbf{N}^{\dagger}\textbf{N}\bar{\psi}d\xi\nonumber\\
&=&-\frac{i}{8\hbar}\sum_e Al_e\int^1_{-1}\bar{\phi}^{\dagger}\sin\left[k\left(x_{e_1}\frac{1-\xi}{2}+x_{e_2}\frac{1+\xi}{2}\right)-\omega t \right]\nonumber\\ 
& &\left[ \begin{array}{cc}
(1-\xi)(1-\xi)& (1-\xi)(1+\xi)\\
(1+\xi)(1-\xi)& (1+\xi)(1+\xi)\\
\end{array}
\right] \bar{\psi}d\xi
\label{time-varying-potential-term}
\end{eqnarray}
Carrying out the integral and simplifying we obtain the element equation
\begin{eqnarray}
&=&\bar{\phi}^{\dagger}\left\{-\frac{iAl_e}{8\hbar} \frac{8}{k^3(x_{e_1}-x_{e_2})^3}\right.\nonumber\\
& &\left.\tiny
\left[ \begin{array}{cc}
(-2+k^2(x_{e_1}-x_{e_2})^2)\cos\left[t\omega-kx_{e_1}\right]+2(\cos\left[t\omega-kx_{e_2}\right]+k(x_{e_1}-x_{e_2})\sin\left[t\omega-kx_{e_1}\right] )& 2(k(x_{e_1}-x_{e_2})\cos\left[\frac{1}{2}k(x_{e_1}-x_{e_2})\right]-2\sin\left[\frac{1}{2}k(x_{e_1}-x_{e_2})\right])\sin\left[t\omega-\frac{1}{2}k(x_{e_1}-x_{e_2})\right]\\
2(k(x_{e_1}-x_{e_2})\cos\left[\frac{1}{2}k(x_{e_1}-x_{e_2})\right]-2\sin\left[\frac{1}{2}k(x_{e_1}-x_{e_2})\right])\sin\left[t\omega-\frac{1}{2}k(x_{e_1}-x_{e_2})\right]&(-2+k^2(x_{e_1}-x_{e_2})^2)\cos\left[t\omega-kx_{e_2}\right]+2(\cos\left[t\omega-kx_{e_1}\right]+k(x_{e_2}-x_{e_1})\sin\left[t\omega-kx_{e_2}\right] )\\
\end{array}
\right]\normalsize \bar{\psi}\right\}
\label{time-varying-potential-term}
\end{eqnarray}
